Constraints on the Progenitor of SN 2010jl and Pre-Existing Hot Dust in its Surrounding Medium

A search for the progenitor of SN~2010jl, an unusually luminous core-collapse supernova of Type~IIn, using pre-explosion {\it Hubble}/WFPC2 and {\it Spitzer}/IRAC images of the region, yielded upper limits on the UV and near-infrared (IR) fluxes from any candidate star. These upper limits constrain the luminosity and effective temperature of the progenitor, the mass of any preexisting dust in its surrounding circumstellar medium (CSM), and dust proximity to the star. A {\it lower} limit on the CSM dust mass is required to hide a luminous progenitor from detection by {\it Hubble}. {\it Upper} limits on the CSM dust mass and constraints on its proximity to the star are set by requiring that the absorbed and reradiated IR emission not exceed the IRAC upper limits. Using the combined extinction-IR emission constraints we present viable $M_d-R_1$ combinations, where $M_d$ and $R_1$ are the CSM dust mass and its inner radius. These depend on the CSM outer radius, dust composition and grain size, and the properties of the progenitor. The results constrain the pre-supernova evolution of the progenitor, and the nature and origin of the observed post-explosion IR emission from SN~2010jl. In particular, an $\eta$~Car-type progenitor will require at least 4~mag of visual extinction to avoid detection by the {\it Hubble}. This can be achieved with dust masses $\gtrsim 10^{-3}$~\msun\ (less than the estimated 0.2-0.5~\msun\ around $\eta$~Car) which must be located at distances of $\gtrsim 10^{16}$~cm from the star to avoid detection by {\it Spitzer}.

==> sn2010jl_table3.tex <==

\begin{deluxetable}{lcccc}
\tabletypesize{\footnotesize}
\tablewidth{0pt}
\tablecaption{The ratio $\kappa_{ext}(a,{\rm V})/\left< \kappa(a,T)\right>$ for different progenitors, dust compositions, and grain radii.\tablenotemark{1}}
\tablehead{
\colhead{} &
\colhead{RSG } &
\colhead{YSG} &
\colhead{LBV cold} &
\colhead{LBV hot} 
  }
 \startdata 
 Silicate &  & & & \\    
 0.01 \mic &    1.82   &   1.19  &   0.34  &  0.019 \\
 0.10 \mic  &   13.7   &   6.67   &   2.41   &  0.78  \\
  1.0 \mic  &    3.347 &     2.89  &    2.60  &    2.55  \\
  \hline \\
 ACAR &  & & & \\
  0.01 \mic   &  2.00  &    1.16  &   0.44  &  0.08  \\
  0.10 \mic  &   6.25   &   3.12  &    1.77  &    1.42  \\
  1.0 \mic  &   1.83   &   1.98  &    2.19  &    2.50  \\
  \enddata
  \tablenotetext{1}{See eq.~(\ref{cond1}). Progenitor temperatures are given in Table~1}
  \label{table:taurat}
\end{deluxetable}

